Generalization Properties of Adversarial Training for $\ell_0$-Bounded Adversarial Attacks

We have widely observed that neural networks are vulnerable to small additive perturbations to the input causing misclassification. In this paper, we focus on the $\ell_0$-bounded adversarial attacks, and aim to theoretically characterize the performance of adversarial training for an important class of truncated classifiers. Such classifiers are shown to have strong performance empirically, as well as theoretically in the Gaussian mixture model, in the $\ell_0$-adversarial setting. The main contribution of this paper is to prove a novel generalization bound for the binary classification setting with $\ell_0$-bounded adversarial perturbation that is distribution-independent. Deriving a generalization bound in this setting has two main challenges: (i) the truncated inner product which is highly non-linear; and (ii) maximization over the $\ell_0$ ball due to adversarial training is non-convex and highly non-smooth. To tackle these challenges, we develop new coding techniques for bounding the combinatorial dimension of the truncated hypothesis class.

==> temp_rest.tex <==
\section{Growth Function of Truncated Inner Product}
\label{sec:trunc-inn-prod-growth}

{\color{red}to be organized, name to be changed, here is when we have no
  maximization over the $\ell_0$ ball yet}

Let $\mT_{d, k} \subset \{-1,1\}^{\reals^d}$ be the class of truncated inner
product functions of the form $T_{\vw,k} : \vx \mapsto \sgn(\langle \vw, \vx
\rangle_k)$, i.e.\ $\mT_{d,k} := \{T_{\vw, k}: \vw \in \reals^d\}$. Here,
$\sgn(u) = +1$ when $u \geq 0$ and $\sgn(u) = -1$ when $u < 0$. For integer $n$,
let 
\begin{equation}
  \label{eq:growth-mT}
  \Pi_{\mT_{d,k}}(n) := \max \{ |\{(T_{\vw, k}(\vx_1), \dots, T_{\vw, k}(\vx_n)): T_{\vw,k} \in \mT_{d,k}\}|: \vx_1, \dots, \vx_n \in \reals^d\},
\end{equation}
be the so called \emph{growth function} associated to the function class
$\mT_{d, k}$.

\begin{prop}
  \label{prop:tip-growth-bound-duplicate} For $n
  > d$, we
  have
  \begin{equation}
    \label{eq:tip-growth-bound}
    \Pi_{\mT_{d,k}}(n) \leq \left( \frac{e n}{d-2k} \right)^{\binom{d}{2k}(d-2k)} \times \left( \frac{e n}{2} \right)^{2\binom{d}{2}}.
  \end{equation}
\end{prop}

\subsection{Proof}

Let $A_1, \dots, A_{\binom{d}{2k}}$ be all the subsets of size $d-2k$ of $[d]$
in an arbitrary but fixed order, and define $\valpha_i= (\alpha_{i,1}, \dots, \alpha_{i,d}), 1 \leq i \leq
\binom{d}{2k}$ be the zero-one vector corresponding to the set $A_i$, i.e.
$\alpha_{i,j}$ is 1 if $j \in A_i$ and zero otherwise. For instance, with $d =
4$ and $k=1$, we have $\valpha_1 = (1,1,0,0)$, $\valpha_2 = (1,0,1,0)$,\dots,  and
$\valpha_6 = (0,0,1,1)$. Moreover, define the vectors $\vbeta_i: 1 \leq i \leq
\binom{d}{2}$ such that for each of them we pick two coordinates in $[d]$, set
the value of the coordinate with smaller index to 1, set the value of the
coordinate with larger index to $-1$, and set the value of other $d-2$
coordinates to zero. For instance, if $d = 4$, we have $\vbeta_1 = (1,-1,0,0)$,
$\vbeta_2 = (1,0,-1,0)$, $\vbeta_3 = (1,0,0,-1)$, \dots, and $\vbeta_6 =
(0,0,1,-1)$.

\begin{lem}
\label{lem:trp-sign-code-duplicate}
  % For $\vw, \vx \in \reals^d$, the value of $\sgn(\langle \vw, \vx \rangle_k)$
  % can be determined by knowing the set of signs $(\sgn(\langle \vw, \vx \odot \valpha_i \rangle):
  % 1 \leq i \leq \binom{d}{2k})$ and the set of signs $(\sgn(\langle \vw, \vx
  % \odot \vbeta_j \rangle): 1 \leq j \leq \binom{d}{2})$.
  % {\color{cyan}new version:
    Assume that $\vw, \vx \in \reals^d$ are given, and
    let $\vu := \vw \odot \vx$. Then,
  for any subset $\mJ \subset [d]$ with $|\mJ| = d-2k$, the value of
  $\sgn(\sum_{j \in \mJ} u_{(j)})$ can be determined by knowing the set of signs $(\sgn(\langle \vw, \vx \odot \valpha_i \rangle):
  1 \leq i \leq \binom{d}{2k})$ and the set of signs $(\sgn(\langle \vw, \vx
  \odot \vbeta_j \rangle): 1 \leq j \leq \binom{d}{2})$. More precisely, for any
  such subset $\mJ$, there exists a function $\psi_{\mJ}$ such that for all
  $\vw, \vx \in \reals^d$, with $\vu = \vw \odot \vx$, we have 
  \begin{equation*}
    \sgn\left(\sum_{j \in \mJ} u_{(j)}\right) = \psi_{\mJ}\left(\left(\sgn(\langle \vw, \vx \odot \valpha_i \rangle):
  1 \leq i \leq \binom{d}{2k}\right), \left(\sgn(\langle \vw, \vx
  \odot \vbeta_j \rangle): 1 \leq j \leq \binom{d}{2}\right)\right).
\end{equation*}
In particular, since $\langle \vw, \vx \rangle_k = \sum_{j\in \mJ_*} u_{(j)}$
with $\mJ_* = \{k+1, \dots, d-k\}$, we have
\begin{equation*}
  \sgn(\langle \vw, \vx \rangle_k) = \psi_{*}\left(\left(\sgn(\langle \vw, \vx \odot \valpha_i \rangle):
  1 \leq i \leq \binom{d}{2k}\right), \left(\sgn(\langle \vw, \vx
  \odot \vbeta_j \rangle): 1 \leq j \leq \binom{d}{2}\right)\right),
\end{equation*}
with $\psi_* = \psi_{\mJ_*}$.
%}
\end{lem}

%{\color{red}[notation:$\odot$]}

\begin{proof}
  %{\color{red}[to be added]} % see gnote
  % 2021-11-03_VC-dimension-of-truncated-inner-product page 2-3.
Fix a subset $\mJ \subset [d]$ with $|\mJ| = d-2k$. Note that for $1 \leq j \leq
\binom{d}{2}$, if $\vbeta_j$ has value 1 at coordinate $a$ and $-1$ at coordinate $b$,
then we have
\begin{equation*}
  \langle \vw, \vx \odot \vbeta_j \rangle = w_a x_a - w_b x_b.
\end{equation*}
Therefore
\begin{equation*}
  \sgn(\langle \vw, \vx \odot \vbeta_j \rangle) =
  \begin{cases}
    1 & w_a x_a \geq w_b x_b  \\
    -1 & \text{otherwise}.
  \end{cases}
\end{equation*}
This means that given $\left(\sgn(\langle \vw, \vx
  \odot \vbeta_j \rangle): 1 \leq j \leq \binom{d}{2}\right)$, we can 
sort the elements in $\vu = \vw \odot \vx$ and obtain an ordering $i_1 \leq
\dots \leq i_d$ such that $u_{i_1} \leq u_{i_2} \leq \dots \leq u_{i_d}$. This
means that
\begin{equation*}
 \sum_{j \in \mJ} u_{(j)}  = \sum_{j \in \mJ} u_{i_j}.
\end{equation*}
But if $\tilde{\mJ} := \{i_j : j \in \mJ\}$, and $\valpha_{i(\tilde{\mJ})}$ is the indicator vector
associated to $\tilde{\mJ}$, we have
\begin{equation*}
  \sgn\left( \sum_{j \in \mJ} u_{(j)} \right) = \sgn\left( \sum_{j \in \tilde{\mJ}} u_j \right) = \sgn\left( \langle \vw, \vx \odot \valpha_{i(\tilde{\mJ})} \rangle  \right),
\end{equation*}
which is known given $\left(\sgn(\langle \vw, \vx \odot \valpha_i \rangle):
  1 \leq i \leq \binom{d}{2k}\right)$. The proof is complete since as was
discussed above, $\tilde{\mJ}$ is a function of $\left(\sgn(\langle \vw, \vx
  \odot \vbeta_j \rangle): 1 \leq j \leq \binom{d}{2}\right)$.
\end{proof}

\begin{proof}[Proof of Proposition~\ref{prop:tip-growth-bound}]
  Fix $\vx_1, \dots, \vx_n \in \reals^d$. With $m := \binom{d}{2k} +
  \binom{d}{2}$, we define the $n \times m$ matrix $M := (\vx_{i,j}: i \in [n],
  j \in [m])$ as follows. For $1 \leq j \leq \binom{d}{2k}$, let $\vx_{i,j} := \vx_i
  \odot \valpha_j$, and for $1+\binom{d}{2k} \leq j \leq m$, let $\vx_{i,j} :=
  \vx_i \odot \vbeta_{j - \binom{d}{2k}}$.

  For $\vw \in \reals^d$, we define the $n \times m$ matrix $M(\vw)$ with $\pm
  1$ entries as follows:
  \begin{equation*}
    M(\vw) :=
    \begin{bmatrix}
      \sgn(\langle \vw, \vx_{1,1} \rangle)  & \dots & \sgn(\langle \vw, \vx_{1,m} \rangle) \\
      \vdots & \ddots & \vdots \\
      \sgn(\langle \vw, \vx_{n,1} \rangle) & \dots & \sgn(\langle \vw, \vx_{n,m} \rangle)
    \end{bmatrix}
  \end{equation*}
Note that from Lemma~\ref{lem:trp-sign-code}, $T_{\vw, k}(\vx_i) = \sgn(\langle
\vw, \vx_i \rangle_k)$ for $1 \leq i \leq n$ are determines by knowing the
matrix $M(\vw)$. Therefore, the total number of configurations for $(T_{\vw,
  k}(\vx_1), \dots, T_{\vw, k}(\vx_n))$ when $T_{\vw, k}$ ranges over $\mT_{d,
  k}$ is bounded from above by the total number of configurations for the matrix
$M(\vw)$ when $\vw$ ranges over $\reals^d$. In other words,
\begin{equation}
  \label{eq:T-vx-1n-bound-M-w}
  |\{(T_{\vw, k}(\vx_1), \dots, T_{\vw, k}(\vx_n)): T_{\vw, k} \in \mT_{d,k}\}| \leq |\{M(\vw): \vw \in \reals^d\}|.
\end{equation}
Moreover, if $M_j(\vw)$ for $1 \leq j \leq m$ denote the $j$th column of
$M(\vw)$, the total number of configurations for $M(\vw)$ is bounded above by
the product of the total number of configurations over all the columns, i.e.\
\begin{equation}
  \label{eq:conf-Mw-bound-prod-columns}
  |\{M(\vw): \vw \in \reals^d\}| \leq \prod_{j=1}^m |\{M_j(\vw): \vw \in \reals^d\}|.
\end{equation}
Note that for $1 \leq j \leq \binom{d}{2k}$, $\vx_{1, j}, \dots, \vx_{n,j}$ are
vectors in a $d-2k$ dimensional subspace of $\reals^d$. This is becasue
$\vx_{i,j} = \vx_i \odot \valpha_j$ and all but $d-2k$ elements in $\valpha_j$
are zero. Consequently, since the VC dimension of the sign of the inner product
in $\reals^{d-2k}$ is $d-2k$, and $n > d$, the Sauer–Shelah lemma
{\color{red}[ref?]} implies that
\begin{equation}
  \label{eq:Mjw-conf-j-alpha}
  |\{M_j(\vw): \vw \in \reals^d\}| \leq \left( \frac{e n}{d-2k} \right)^{d-2k} \qquad \text{ for } 1 \leq j \leq \binom{d}{2k}.
\end{equation}
Using a similar argument, since $\vx_{1,j}, \dots, \vx_{n,j}$ are vectors in a
$2$ dimensional subspace of $\reals^d$,  we have
\begin{equation}
  \label{eq:Mjw-conf-j-beta}
  |\{M_j(\vw): \vw \in \reals^d\}| \leq \left( \frac{e n}{2} \right)^{2} \qquad \text{ for } 1+\binom{d}{2k} \leq j \leq m.
\end{equation}
Substituting~(\ref{eq:Mjw-conf-j-alpha}) and (\ref{eq:Mjw-conf-j-beta})
back into~(\ref{eq:conf-Mw-bound-prod-columns}) and combining
with~(\ref{eq:T-vx-1n-bound-M-w}), we realize that
\begin{equation*}
  |\{(T_{\vw, k}(\vx_1), \dots, T_{\vw, k}(\vx_n)): T_{\vw, k} \in \mT_{d,k}\}| \leq \left( \frac{e n}{d-2k} \right)^{\binom{d}{2k}(d-2k)} \times \left( \frac{e n}{2} \right)^{2\binom{d}{2}}.
\end{equation*}
Since the same bound  holds for all $\vx_1, \dots, \vx_n$, we get
\begin{align*}
  \Pi_{\mT_{d,k}}(n) &= \max \{ |\{(T_{\vw, k}(\vx_1), \dots, T_{\vw, k}(\vx_n)): T_{\vw,k} \in \mT_{d,k}\}|: \vx_1, \dots, \vx_n \in \reals^d\} \\
                     &\leq \left( \frac{e n}{d-2k} \right)^{\binom{d}{2k}(d-2k)} \times \left( \frac{e n}{2} \right)^{2\binom{d}{2}}.
  \end{align*}
This completes the proof.
\end{proof}


\section{Maximization over the $\ell_0$ ball}
\label{sec:max-l0}

Let $\tmT_{d,k} \subset \{-1,+1\}^{\reals^d \times \{\pm 1\}}$  be the class of
functions $\tT_{\vw, k}$ parametrized by $\vw \in \reals^d$ defined as
\begin{equation*}
  \tT_{\vw, k}(\vx, y) := \max_{\vxp \in \mB_0(\vx, k)} \one{y \neq \sgn(\langle \vw, \vxp \rangle_k)},
\end{equation*}
for $\vx \in \reals^d$ and $y \in \{\pm 1\}$.
Our goal in this section is to bound the growth function of this function class,
i.e.\
\begin{equation*}
  \Pi_{\tmT_{d,k}}(n) = \max\{|\{(\tT_{\vw, k}(\vx_1, y_1), \dots, \tT_{\vw, k}(\vx_n, y_n)): \tT_{\vw, k} \in \tmT_{d,k}\}|: \vx_1, \dots, \vx_n \in \reals^d, y_1, \dots, y_n \in \{\pm 1\}\}.
\end{equation*}
\begin{prop}
  \label{prop:max-l0-growth-bound-duplicate}
  For $n > d$, we have
  \begin{equation*}
    \Pi_{\tmT_{d,k}}(n) \leq 1 + \left( \frac{e n}{d-2k} \right)^{\binom{d}{2k}(d-2k)} \times \left( \frac{e n}{2} \right)^{2\binom{d}{2}}.
  \end{equation*}
\end{prop}

Before giving the proof, We first explain our proof strategy and state some
lemmas.
In order to bound $\Pi_{\tmT_{d,k}}(n)$, observe that we may write
\begin{equation}
  \label{eq:tT-max-1-I1-I2-duplicate}
  \begin{aligned}
    \tT_{\vw, k}(\vx, y) &= \one{\exists \vxp \in \mB_0(\vx, k): y \neq \sgn(\langle \vw, \vxp \rangle_k)} \\
    &= \one{\sgn(\langle \vw, \vx \rangle_k) \neq y} \vee \one{\exists \vxp \in \mB_0(\vx, k): \sgn(\langle \vw, \vxp \rangle_k) \neq \sgn(\langle \vw, \vx \rangle_k)},
  \end{aligned}
\end{equation}
where $\vee$ denotes logical OR. Our strategy is to bound the growth functions
of each of the two function classes parametrized by $\vw \in \reals^d$ in the right hand side. The growth function of the first
term $\one{\sgn(\langle \vw, \vx \rangle_k) \neq y}$ directly follow from
Proposition~\ref{prop:tip-growth-bound}. Let us denote the second term by
$I_1(\vw, \vx)$,
\begin{equation}
  \label{eq:I1-def-exists-vxp-different-sign-duplicate}
  I_1(\vw, \vx) := \one{\exists \vxp \in \mB_0(\vx, k): \sgn(\langle \vw, \vxp \rangle_k) \neq \sgn(\langle \vw, \vx \rangle_k))}.
\end{equation}
In order to evaluate $I_1(\vw, \vx)$, it suffices to know the minimum and
maximum values of $\sgn(\langle \vw, \vxp \rangle_k)$ when $\vxp$ ranges in
$\mB_0(\vx, k)$. Note that $\langle \vw, \vx \rangle_k = \tsum_k(\vw \odot
\vx)$, $\langle \vw, \vxp \rangle_k = \tsum_k(\vw \odot \vxp)$,
and 
\begin{equation}
  \label{eq:vxp-vx-k-implies-vw-odot-vxp-vw-odot-vx}
  \snorm{\vxp - \vx}_0 \leq k \qquad \text{ implies } \qquad \snorm{\vw
  \odot \vx - \vw \odot \vxp}_0 \leq k.
\end{equation}
This motivates the following Lemma.

\begin{lem}
\label{lem:tsum-l0-min-max-old-long}
  Let $\vu \in \reals^d$. Then, for any $\vup \in \reals^d$ such that
  $\snorm{\vu - \vup}_0 \leq k$, we have
  \begin{equation*}
    u_{{(1)}} + u_{(2)} + \dots + u_{(d-2k)} \leq \tsum_k(\vup) \leq u_{(2k+1)} + u_{(2k+2)} + \dots + u_{(d)}.
  \end{equation*}
  Moreover, the inequalities on both sides are attainable. 
More precisely, if $u_{i_1} \leq u_{i_2} \leq \dots \leq u_{i_d}$ is an ordering of
coordinates in $\vu$, the upper bound is attained by setting the $k$ smallest
coordinates to be bigger than the largest value $u_{(d)}$, i.e.\
\begin{align*}
  &u'_{i_1} = u'_{i_2} = \dots =u'_{i_k} = u_{(d)} + 1 \\
  &u'_{i_j} = u_{i_j} \qquad \text{for } j > k,
\end{align*}
and the lower bound is attained by setting the $k$ largest coordinates to be
smaller than the smallest value $u_{(1)}$, i.e.\
 \begin{align*}
   &u'_{i_{d-k+1}} = u'_{i_{d-k+2}} = \dots =u'_{i_d} = u_{(1)} -1 \\
   &u'_{i_j} = u_{i_j} \qquad \text{for } j \leq d-k.
 \end{align*}
Hence,
  \begin{equation}
    \label{eq:min-max-tsum-over-ell0-ball}
    \begin{aligned}
      \min\{\tsum_k(\vup): \vup \in \mB_0(\vu, k)\} &= u_{(1)} + \dots + u_{(d-2k)} \\
      \max\{\tsum_k(\vup): \vup \in \mB_0(\vu, k)\} &= u_{(2k+1)} + \dots + u_{(d)} 
    \end{aligned}
  \end{equation}
\end{lem}

Note that from~\eqref{eq:vxp-vx-k-implies-vw-odot-vxp-vw-odot-vx}, we have $\{\vw \odot \vxp: \vxp \in \mB_0(\vx, k)\} \subset
\mB_0(\vw \odot \vx, k)$. Therefore, Lemma~\ref{lem:tsum-l0-min-max} readily implies that with $\vu := \vw \odot \vw$,
we have
\begin{equation*}
  \inf\{\langle \vw, \vxp \rangle_k : \vxp \in \mB_0(\vx, k)\} \geq u_{(1)} + \dots + u_{(d-2k)},
\end{equation*}
and
\begin{equation*}
  \sup\{\langle \vw, \vxp \rangle_k : \vxp \in \mB_0(\vx, k)\} \leq u_{(2k+1)} + \dots + u_{(d)}.
\end{equation*}
However, the two sets $\{\vw \odot \vxp: \vxp \in \mB_0(\vx, k)\}$ and
$\mB_0(\vw \odot \vx, k)$ might be  different and the inequalities above might
not be strict. The reason
is that when $w_i = 0$ for some $i \in [d]$, then $w_i x'_i = w_i x_i = 0$ even
if $x'_i \neq x_i$, i.e.\ we can not perturb the $i$th coordinate in $\vw \odot
\vx$. Despite this, the following Lemma shows that if the number of zero
coordinates in $\vw$ is bigger than $k$, then we can predict the value of  $I_1(\vw, \vx)$
from the signs of the above bounds, even though bounds might not be tight. 
\begin{lem}
  \label{lem:Aw-large-k-I1-I2-duplicate}
  Assume that $\vw \in \reals^d$ is given such that $|\{i \in [d]: w_i \neq 0\}| > k$. Then,
  for all $\vx \in \reals^d$, we have 
  \begin{equation*}
    I_1(\vw, \vx) =    \one{\sgn(u_{(1)} + \dots + u_{(d-2k)}) \neq \sgn(u_{(2k+1)} + \dots u_{(d)})} =: I_2(\vw, \vx),
  \end{equation*}
  where $\vu = \vw \odot \vx$.
\end{lem}
Additionally, if $|\{i \in [d]: w_i \neq 0\}| \leq k$, $\langle \vw, \vxp \rangle_k$
is always zero:
\begin{lem}
\label{lem:vw-at-most-k-nonzero-trp-zero-duplicate}
  Assume that $\vw \in \reals^d$ is given such that $|\{i \in [d]: w_i \neq 0\}| \leq k$. Then, for
  all $\vx \in \reals^d$, we have $\langle \vw,
  \vx \rangle_k = 0$.
\end{lem}


%\vspace{5cm}





\begin{proof}[Proof of Proposition~\ref{prop:max-l0-growth-bound}]
%   Observe that
%   \begin{align*}
%     \max_{\vxp \in \mB_0(\vx, k)} \one{y \neq \sgn(\langle \vw, \vxp \rangle_k)} &= \one{\exists \vxp \in \mB_0(\vx, k): y \neq \sgn(\langle \vw, \vxp \rangle_k)} \\
%     &= \one{\sgn(\langle \vw, \vx \rangle_k) \neq y} \vee \one{\exists \vxp \in \mB_0(\vx, k): \sgn(\langle \vw, \vxp \rangle_k) \neq \sgn(\langle \vw, \vx \rangle_k)},
%   \end{align*}
% where $\vee$ denotes logical OR. 
%   {\color{red}[do I want to explain it more? I think it is fine for now.
%     $\vee$]}
%   Consequently, we have
%   \begin{equation}
%     \label{eq:pi-tt-pi-F-pi-G}
%     \Pi_{\tmT_{d, k}}(n) \leq \Pi_{\mF}(n) \times \Pi_{\mG}(n),
%   \end{equation}
%   where $\mF:= \{f_{\vw}: \reals^d \times \{\pm 1\} \rightarrow \{\pm 1\}\}$  is
%   the class of functions $f_{\vw}$ parametrized by $\vw \in \reals^d$ defied as
%   \begin{equation*}
%     f_{\vw}(\vx, y) := \one{\sgn(\langle \vw, \vx \rangle_k) \neq y},
%   \end{equation*}
%   and $\mG:= \{g_{\vw}: \reals^d \rightarrow \{\pm 1\}\}$ is the class of
%   functions $g_{\vw}$ parametrized by $\vw \in \reals^d$ defined as
%   \begin{equation*}
%     g_{\vw}(\vx) := \one{\exists \vxp \in \mB_0(\vx, k): \sgn(\langle \vw, \vxp \rangle_k) \neq \sgn(\langle \vw, \vx \rangle_k)}.
%   \end{equation*}
%   We now bound each of the two growth functions $\Pi_{\mF}(n)$ and $\Pi_{\mG}(n)$
%   and substitute them into~(\ref{eq:pi-tt-pi-F-pi-G}) to bound
%   $\Pi_{\tmT_{d,k}}(n)$.
%   We begin by bounding $\Pi_{\mF}(n)$. It is straightforward to see that
%   $\Pi_{\mF}(n) = \Pi_{\mT_{d,k}}(n)$ ({\color{red}[perhaps give ref to the
%     previous part this was defined and discussed when things are organized]}
%   {\color{orange}[maybe give a short sentence about this, e.g. that the only
%     difference between $\mF$ and $\mT_{d, k}$ is the existence of $y$ which
%     possibly negates the sign of each coordinate and hence does not change the
%     number of configurations.]}).
%   Therefore, using Proposition~\ref{prop:tip-growth-bound}, for $n \geq d$, we have
%   \begin{equation}
%     \label{eq:Pi-mF-bound}
%     \Pi_{\mF}(n) \leq \left( \frac{e n}{d-2k} \right)^{\binom{d}{2k}(d-2k)} \times \left( \frac{e n}{2} \right)^{2\binom{d}{2}}.
%   \end{equation}
%   Next, we study $\Pi_{\mG}(n)$. Note that 
Fix $\vx_1, \dots, \vx_n \in \reals^d$ and $y_1, \dots, y_n \in \{\pm 1\}$. From
Lemma~\ref{lem:vw-at-most-k-nonzero-trp-zero}, if $|\{i \in [d]: w_i \neq 0\}|
\leq k$, we have $\langle \vw, \vx'_i \rangle_k = 0$ for all $\vx'_i \in
\mB_0(\vx, k)$ and $1 \leq i \leq n$. This means that $\tT_{\vx, k}(\vx_i, y_i)
= \one{y_i = -1}$. Thereby,
\begin{equation}
  \label{eq:conf-count-tT-1+-bound}
  |\{(\tT_{\vw, k}(\vx_1, y_1), \dots, \tT_{\vw, k}(\vx_n, y_n)): \tT_{\vw, k} \in \tmT_{d,k}\}| \leq 1 +   |\{(\tT_{\vw, k}(\vx_1, y_1), \dots, \tT_{\vw, k}(\vx_n, y_n)): \vw \in \mW_{>k}\}|, 
\end{equation}
where
\begin{equation*}
  \mW_{> k} := \{\vw \in \reals^d: |\{i \in [d]: w_i \neq 0\}| > k\}.
\end{equation*}
But from~\eqref{eq:tT-max-1-I1-I2-1} and Lemma~\ref{lem:Aw-large-k-I1-I2}, for
$\vw \in \mW_{>k}$ and $1 \leq i \leq n$, we have
\begin{equation*}
  \tT_{\vw, k}(\vx_i, y_i) = \one{\sgn(\langle \vw, \vx_i \rangle_k) \neq y_i} \vee \one{\sgn(u^{(i)}_{(1)} + \dots + u^{(i)}_{(d-2k)}) \neq \sgn(u^{(i)}_{(2k+1)} + \dots u^{(i)}_{(d)})},
\end{equation*}
where $\vu^{(i)} := \vw \odot \vx_i$. Note that all the sign terms in the above
expression are of the form $\sgn(\sum_{j \in \mJ}(u^{(i)}_j))$ for some $\mJ
\subset [d]$ with $|\mJ| = d-2k$. Specifically, with $\mJ_1 := \{k+1, \dots,
d-k\}$, $\mJ_2:= \{1, \dots, d-2k\}$, and $\mJ_3 := \{2k+1, \dots, d\}$, we have
\begin{align*}
  \sgn(\langle \vw, \vx_i \rangle_k) &= \sgn\left( \sum_{j \in \mJ_1} u^{(i)}_j  \right) \\
  \sgn(u^{(i)}_{(1)} + \dots + u^{(i)}_{(d-2k)}) &= \sgn\left( \sum_{j \in \mJ_2}u^{(i)}_j \right)\\
  \sgn(u^{(i)}_{(2k+1)} + \dots u^{(i)}_{(d)}) &= \sgn\left( \sum_{j \in \mJ_3}u^{(i)}_j \right).
\end{align*}
Thereby, Lemma~\ref{lem:trp-sign-code} implies that all of these sign terms are
functions of $(\sgn(\langle \vw, \vx_{i,j} \rangle): 1 \leq j \leq m)$ where $m
= \binom{d}{2k} + \binom{d}{2}$, for $1 \leq j \leq \binom{d}{2k}$, $\vx_{i,j} =
\vx_i \odot \valpha_j$, and for $1 + \binom{d}{2k} \leq j \leq m$, $\vx_{i,j} =
\vx_i \odot \vbeta_{j - \binom{d}{2k}}$. Therefore, we may employ a proof
strategy  similar to that of Proposition~\ref{prop:tip-growth-bound}. More
precisely, for $\vw \in \mW_{>k}$, we define the $n \times m$ matrix $M(\vw)$ with $\pm
  1$ entries as follows:
  \begin{equation*}
    M(\vw) :=
    \begin{bmatrix}
      \sgn(\langle \vw, \vx_{1,1} \rangle)  & \dots & \sgn(\langle \vw, \vx_{1,m} \rangle) \\
      \vdots & \ddots & \vdots \\
      \sgn(\langle \vw, \vx_{n,1} \rangle) & \dots & \sgn(\langle \vw, \vx_{n,m} \rangle)
    \end{bmatrix}
  \end{equation*}
  The above discussion implies that
  \begin{equation}
    \label{eq:tT-conf-count-mW-big-k-Mw-bound}
    |\{(\tT_{\vw, k}(\vx_1, y_1), \dots, \tT_{\vw, k}(\vx_n, y_n)): \vw \in \mW_{>k}\}| \leq |\{M(\vw): \vw \in \mW_{> k}\}| \leq |\{M(\vw): \vw \in \reals^d\}|.
  \end{equation}
  But as we saw in the proof of Proposition~\ref{prop:tip-growth-bound}, since
  $n > d$, we have
  \begin{equation*}
    |\{M(\vw): \vw \in \reals^d\}| \leq \left( \frac{e n}{d-2k} \right)^{\binom{d}{2k}(d-2k)} \times \left( \frac{e n}{2} \right)^{2\binom{d}{2}}.
  \end{equation*}
  Comparing this with~\eqref{eq:tT-conf-count-mW-big-k-Mw-bound}
  and~\eqref{eq:conf-count-tT-1+-bound}, we realize that
  \begin{equation*}
    |\{(\tT_{\vw, k}(\vx_1, y_1), \dots, \tT_{\vw, k}(\vx_n, y_n)): \tT_{\vw, k} \in \tmT_{d,k}\}| \leq 1 + \left( \frac{e n}{d-2k} \right)^{\binom{d}{2k}(d-2k)} \times \left( \frac{e n}{2} \right)^{2\binom{d}{2}}.
  \end{equation*}
  Since this bound holds for all $\vx_1, \dots, \vx_n$ and $y_1, \dots, y_n$, we
  realize that
  \begin{align*}
    \Pi_{\tmT_{d,k}}(n) &= \max\{|\{(\tT_{\vw, k}(\vx_1, y_1), \dots, \tT_{\vw, k}(\vx_n, y_n)): \tT_{\vw, k} \in \tmT_{d,k}\}|: \vx_1, \dots, \vx_n \in \reals^d, y_1, \dots, y_n \in \{\pm 1\}\} \\
    &\leq 1 + \left( \frac{e n}{d-2k} \right)^{\binom{d}{2k}(d-2k)} \times \left( \frac{e n}{2} \right)^{2\binom{d}{2}}.
  \end{align*}
  This completes the proof.
\end{proof}

\pagebreak

% \begin{equation*}
%   I_1(\vw, \vx) := \one{\exists \vxp \in \mB_0(\vx, k): \sgn(\langle \vw, \vxp \rangle_k \neq \sgn(\langle \vw, \vx \rangle_k)}.
% \end{equation*}

% With $\vu := \vw \odot \vx$
% \begin{equation*}
%   I_2(\vw, \vx) := \one{\sgn(u_{(1)} + \dots + u_{(d-2k)}) \neq \sgn(u_{(2k+1)} + \dots u_{(d)})}.
% \end{equation*}


% With $\vu := \vw \odot \vx$, order ascending





\begin{proof}[Proof of Lemma~\ref{lem:vw-at-most-k-nonzero-trp-zero}]
  Recalling the definition of $A_{\vw}$, the assumption $|A_{\vw}| \leq k$ means
  that all but at most $k$ elements in $\vw$ are zero. This implies that all but
  at most $k$ elements of $\vw \odot \vx$ are also zero, and there are at least
  $d-k$ zero elements in $\vw \odot \vx$. Therefore, since there are no more
  than $k$  nonzero elements, after truncation, they will be removed and only
  zero elements will survive. This means $\langle \vw, \vx \rangle_k =
  \tsum_k(\vw \odot \vx) = 0$.
\end{proof}

\appendix

\section{Proof of Proposition~\ref{prop:max-l0-growth-bound}}
\label{app:prop-max-l0-growth-proof}

The following Lemma~\ref{lem:order-vector-equivalent} gives
an equivalent form for the quantities $u_{(i)}$, $1 \leq i \leq d$. The proof of
Lemma~\ref{lem:order-vector-equivalent}   is
straightforward and hence is omitted. 


\begin{lem}
  \label{lem:order-vector-equivalent-duplicate}
  Given $\vu = (u_1, \dots, u_d) \in \reals^d$, for $1 \leq i \leq d$, we have
  \begin{equation*}
    u_{(i)} = \min \{\alpha: |\{1 \leq j \leq d: u_j \leq \alpha\}| \geq i\}.
  \end{equation*}
\end{lem}

\begin{lem}
\label{lem:up-k+1-u-i-duplicate}
  Assume that $\vu, \vup \in \reals^d$ are given such that $\snorm{\vu - \vup}_0
  \leq k$. Then for $1 \leq i \leq d -k$, we have
  \begin{equation*}
    u'_{(k+i)} \geq u_{(i)}.
  \end{equation*}
\end{lem}

\begin{proof}[Proof of Lemma~\ref{lem:up-k+1-u-i}]
 Fix $1 \leq i \leq d-k$. Using Lemma~\ref{lem:order-vector-equivalent} above,
 we have
 \begin{equation*}
   u'_{(k+i)} = \min \{\alpha: |\{1 \leq j \leq d: u'_j \leq \alpha\}| \geq k+i\}.
 \end{equation*}
 Let $\alpha^*$ be the minimum in the right hand side. Note that  there are at least $k+i$
 coordinates in $\vup$ with values no more than $\alpha^*$, let $1\leq j_1 <
 \dots <  j_{k+i} \leq d$ be the index of such coordinates. Since $\snorm{\vu -
   \vup}_0\leq k$, all the
 coordinates except for at most $k$ of them in $\vup$ are identical to $\vu$.
 Therefore, the value of $\vu$ and $\vup$ are different in at most $k$ of the
 indices $j_1, \dots, j_{k+1}$. Consequently, there are at least $i$
 coordinates in $j_1, \dots, j_{k+i}$ where $\vup$ and $\vu$ match. Thereby
 \begin{equation*}
   u_{(i)} = \min\{\beta: |\{1 \leq j \leq d: x_j \leq \beta\}| \geq i\} \leq \alpha^* = u'_{(k+i)},
 \end{equation*}
 which completes the proof.
\end{proof}

\begin{proof}[Proof of Lemma~\ref{lem:tsum-l0-min-max}]
  Using Lemma~\ref{lem:up-k+1-u-i}, we may write
  \begin{align*}
    \tsum_k(\vup) &= \sum_{i=k+1}^{d-k} u'_{(i)} \\
                  &= \sum_{i=1}^{d-2k} u'_{(k+i)} \\
    &\geq \sum_{i=1}^{d-2k} u_{(i)},
  \end{align*}
  which is the desired lower bound. On the other hand, since $\snorm{\vup -
    \vu}_0 = \snorm{\vu - \vup}_0 \leq k$, using Lemma~\ref{lem:up-k+1-u-i} after
  swapping the role of $\vu$ and $\vup$, we get
  \begin{align*}
    u_{(2k+1)} + \dots + u_{(d)} &= \sum_{i=k+1}^{d-k} u_{(k+i)} \\
                                 &\geq \sum_{i=k+1}^{d-k} u'_{(i)} \\
    &= \tsum_k(\vup),
  \end{align*}
  which is precisely the desired upper bound.

  Now let $u_{i_1} \leq \dots \leq u_{i_d}$ be an ordering of $\vu$ and let
  $\vup \in \mB_0(\vu, k)$ be such that
\begin{align*}
  &u'_{i_1} = u'_{i_2} = \dots =u'_{i_k} = u_{(d)} + 1 \\
  &u'_{i_j} = u_{i_j} \qquad \text{for } j > k.
\end{align*}
Clearly, the largest $k$ values of $\vup$ are $u_{(d)}+1$ which correspond to
coordinates $i_1, \dots, i_k$. Furthermore, the smallest $k$ values of $\vup$
are $u'_{i_{k+j}} = u_{i_{k+j}} = u_{(k+j)}$ for $1 \leq j \leq k$.
Consequently, after truncating the $k$ largest and the $k$ smallest values in
$\vup$, we get
\begin{equation*}
  \tsum_k(\vup) = u'_{i_{2k+1}} + \dots + u'_{i_d} = u_{i_{2k+1}} + \dots + u_{i_d} = u_{(2k+1)} + \dots + u_{(d)}.
\end{equation*}
Hence, $\vup$ attains the upper bound. Similarly, the vector $\vup \in
\mB_0(\vu, k)$ such that
 \begin{align*}
   &u'_{i_{d-k+1}} = u'_{i_{d-k+2}} = \dots =u'_{i_d} = u_{(1)} -1 \\
   &u'_{i_j} = u_{i_j} \qquad \text{for } j \leq d-k,
 \end{align*}
attains the lower bound. Hence, the inequalities are sharp and are in fact the
minimum and the maximum of $\tsum_k(\vup)$ as $\vup$ ranges over $\mB_0(\vu,
k)$. This completes the proof.
\end{proof}

Given $\vw \in \reals^d$, we define
\begin{equation*}
  \admiss_{\vw} := \{i \in [d]: w_i \neq 0\},
\end{equation*}
and $\admiss_{\vw}^c := [d] \setminus \admiss_{\vw}$.
Moreover, given $\vx \in \reals^d$, let $\vu = \vw \odot \vx$. We may order the
coordinates in $\vu$ in an ascending order 
\begin{equation}
\label{eq:u-vw-vx-order-i1-id}
  u_{i_1} \leq u_{i_2} \leq \dots \leq u_{i_d}.
\end{equation}
Note that indeed $u_{i_j} = u_{(j)}$ for $j \in [d]$.
Assume that  $\admiss_{\vw}^c \neq \emptyset$. In this case, note that for $i \in
\admiss_{\vw}^c$, we have $u_i = x_i w_i = 0$. Hence, we may choose the above
permutation $i_1, \dots, i_d$ such that the indices in $\admiss_{\vw}^c$ are
grouped together, i.e.\ for some $1 \leq a \leq b \leq d$, we have 
\begin{equation}
\label{eq:u-vw-vx-order-Awc-ab}
  \admiss_{\vw}^c = \{i_a, i_{a+1}, \dots, i_b\}.
\end{equation}

\begin{definition}
  \label{def:good-order}
We say that an ordering $i_1, \dots, i_d$ of the coordinates in $\vu = \vw \odot \vx$ is good
if~\eqref{eq:u-vw-vx-order-i1-id} holds, and  if $A_{\vx}^c \neq \emptyset$,
then \eqref{eq:u-vw-vx-order-Awc-ab} holds for some $1 \leq a \leq b \leq d$.
\end{definition}

\begin{lem}
  \label{lem:inf-sup-w-x-k-equality-cond-duplicate}
  Assume that  $\vw, \vx \in \reals^d$ are given and define $\vu := \vw \odot \vx$.
  \begin{enumerate}
  \item We have 
    \begin{equation*}
      \inf\{\langle \vw, \vxp \rangle_k: \vxp \in \mB_0(\vx, k)\} \geq u_{(1)} + \dots +u_{(d-2k)}.
    \end{equation*}
    Moreover,  if $w_i \neq 0$ for all $i \in [d]$, or $|\{i: u_i \geq 0
    \text{ and } w_i \neq 0\}| \geq k$, then the infimum is minimum and equality
    holds. 
  \item We have 
    \begin{equation*}
      \sup\{\langle \vw, \vxp \rangle_k: \vxp \in \mB_0(\vx, k)\} \leq u_{(2k+1)} + \dots +u_{(d)}.
    \end{equation*}
    Moreover,  if $w_i \neq 0$ for all $i \in [d]$, or $|\{i: u_i \leq 0
    \text{ and } w_i \neq 0\}| \geq k$, then the supremum is maximum and
    equality holds.
  \end{enumerate}
\end{lem}

\begin{proof}[Proof of Lemma~\ref{lem:inf-sup-w-x-k-equality-cond}]
  %{\color{red}[to be added, see gtag ``2022-01-28 15-41-30'']}
  We give the proof of the lower bound (part 1). The proof of the upper bound
  (part 2) is similar and hence is omitted.
  % In fact, it is obtained by replacing $\vw$ with $-\vw$.
  Note that
  \begin{equation*}
    \{\vw \odot \vxp: \vxp \in \mB_0(\vx, k)\} \subset \mB_0(\vu, k). 
  \end{equation*}
  Therefore, Lemma~\ref{lem:tsum-l0-min-max} implies that
  \begin{equation}
    \label{eq:inf-wxp-u1-proof-1}
  \begin{aligned}
    \inf\{\langle \vw, \vxp \rangle_k: \vxp \in \mB_0(\vx, k)\} &\geq  \min \{\tsum_k(\vup): \vup \in \mB_0(\vu, k)\} \\
    &= u_{(1)} + \dots + u_{(d-2k)}.
  \end{aligned}
  \end{equation}
  On the other hand, if $w_i \neq 0$ for all $i \in [d]$, or equivalently if
  $|\admiss_{\vw}^c| = 0$, we have $\{\vw \odot
  \vxp: \vxp \in \mB_0(\vx, k)\} \subset \mB_0(\vu, k)$ and
  indeed~\eqref{eq:inf-wxp-u1-proof-1} becomes inequality. Now we show that if
  $|\admiss_{\vw}^c| \neq 0$ and $|\{i: u_i \geq 0 \text{ and } w_i \neq 0\}|
  \geq k$, then the inequality also becomes equality. In order to show this, let
  \begin{equation*}
    u_{i_1} \leq u_{i_2} \leq \dots \leq u_{i_d},
  \end{equation*}
  be an ordering of the coordinates in $\vu$ in ascending order. Note that since
  $\{i: u_i \geq 0, w_i \neq 0\}| \geq k$, we can choose  the  ordering so
  that the coordinates corresponding to the top $k$ elements fall in
  $\admiss_{\vw}$, i.e.
  \begin{equation}
    \label{eq:i-d-k+1-id-in-admiss}
    \{i_{d-k+1}, \dots, i_d\} \subseteq \admiss_{\vw}.
  \end{equation}
  Now, define $\vxp \in \mB_0(\vx, k)$ as follows. For $d - k +1 \leq j \leq d$,
  let $x'_{i_j}$ be such that $w_{i_j} x'_{i_j} = u_{(1)} - 1$. Note that this
  is doable since due to~\eqref{eq:i-d-k+1-id-in-admiss}, we have $w_{i_j} \neq
  0$ for $d - k +1 \leq j \leq d$. On the other hand, for $j \leq d -k$, let
  $x'_{i_j} = x_{i_j}$. Note that with this specific perturbation, the $k$
  minimum values in $\vw \odot \vxp$ are
  precisely the coordinates $i_{d-k+1}, \dots, i_d$. Therefore
  \begin{equation*}
    \langle \vw, \vxp \rangle_k = \tsum_k(\vw \odot \vxp) = u_{(1)} + \dots u_{(d-2k)},
  \end{equation*}
  and hence~\eqref{eq:inf-wxp-u1-proof-1} becomes equality.
\end{proof}

\begin{proof}[Proof of Lemma~\ref{lem:Aw-large-k-I1-I2}]
  %{\color{red}[to be added, see gtag ``2022-01-28 18-38-33'']}
  Let $\vu = \vw \odot \vx$ and 
  \begin{equation*}
    u_{i_1} \leq u_{i_2} \leq \dots \leq u_{i_d},
  \end{equation*}
  be an ordering of the coordinates in $\vu$.  
 We divide the proof into cases, based on the sign
  of $u_{i_{k+1}} = u_{(k+1)}$ and $u_{i_{d-k}} = u_{(d-k)}$.

  \underline{Case 1: $u_{i_{k+1}} < 0$ and $u_{i_{d-k}} \leq 0$.} We have
  \begin{equation*}
    \langle \vw, \vx \rangle_k = \tsum_k(\vw \odot \vx) = u_{i_{k+1}} + \dots + u_{i_{d-k}} < 0.
  \end{equation*}
  This means that
  \begin{equation}
    \label{eq:case-1-I1-exists-positive}
    I_1(\vw, \vx)= \one{\exists \vxp \in \mB_0(\vx, k): \langle \vw, \vxp \rangle_k \geq 0}.
  \end{equation}
  On the other hand, note that $u_{i_{k+1}} < 0$ implies that $u_{i_1} , \dots,
  u_{i_k} < 0$. Since for all $i \in [d]$, we have $u_{i} = w_{i} x_{i}$, this means $w_{i_1}, \dots, w_{i_k}\neq 0$ and
  \begin{equation*}
    |\{i:u_i \leq 0, w_i \neq 0 \}| \geq |\{i_1, \dots, i_k\}| = k.
  \end{equation*}
  Therefore, Lemma~\ref{lem:inf-sup-w-x-k-equality-cond} implies that
  \begin{equation*}
    \max\{\langle \vw, \vxp \rangle_k: \vxp \in \mB_0(\vx, k)\}= u_{(2k+1)} + \dots + u_{(d)}.
  \end{equation*}
  Combining this with~\eqref{eq:case-1-I1-exists-positive}, we realize that
  \begin{equation}
    \label{eq:case-1-I1-one-2k+1-d-g-0}
  I_1(\vw, \vx) = \one{u_{(2k+1)} + \dots + u_{(d)} \geq 0}.
  \end{equation}
  Furthermore, since $u_{(d-2k)} \leq u_{(d-k)} = u_{i_{d-k}} \leq 0$, we have
  $u_{(1)}, \dots, u_{(d-2k)} \leq 0$. But $u_{(1)} \leq u_{(k+1)} = u_{i_{k+1}}
  < 0$. Thereby
  \begin{equation*}
    u_{(1)} + \dots + u_{(d-2k)} < 0.
  \end{equation*}
  Consequently,
  \begin{equation*}
    \one{u_{(2k+1)} + \dots + u_{(d)} \geq 0} = \one{\sgn(u_{(1)} + \dots + u_{(d-2k)}) \neq \sgn(u_{(2k+1)} + \dots + u_{(d)})} = I_2(\vw, \vx).
  \end{equation*}
  Combining this with~\eqref{eq:case-1-I1-one-2k+1-d-g-0}, we realize that
  $I_1(\vw, \vx) = I_2(\vw, \vx)$.

  \underline{Case 2: $u_{i_{k+1}} < 0$ and $u_{i_{d-k}} > 0$.} Note that for $1
  \leq j \leq k$, we have 
  $u_{i_j} \leq u_{i_{k+1}} < 0$. Also, since $u_i = w_i x_i$  for all $i\in
  [d]$, this means $w_{i_j} \neq 0$ for $1 \leq j \leq k$. Thereby
  \begin{equation*}
    |\{i:u_i \leq 0, w_i \neq 0\}| \geq |\{i_1, \dots, i_k\}| = k.
  \end{equation*}
  Consequently, Lemma~\ref{lem:inf-sup-w-x-k-equality-cond} implies that
  \begin{equation}
    \label{eq:case-2-max-u}
    \max\{\langle \vw, \vxp \rangle_k: \vxp \in \mB_0(\vx, k)\} = u_{(2k+1)} + \dots + u_{(d)}.
  \end{equation}
  Likewise, $u_{i_{d-k}} > 0$ implies that for $d-k+1 \leq j \leq d$, we
  have $u_{i_j} > 0$ and $w_{i_j} \neq 0$. Hence,
  \begin{equation*}
    |\{i: u_i \geq 0, w_i \neq 0\}| \geq |\{i_{d-k+1}, \dots, i_d\}| = k,
  \end{equation*}
  and from Lemma~\ref{lem:inf-sup-w-x-k-equality-cond} we have
  \begin{equation}
    \label{eq:case-2-min-u}
    \min\{\langle \vw, \vxp \rangle_k: \vxp \in \mB_0(\vx, k)\} = u_{(1)} + \dots + u_{(d-2k)}.
  \end{equation}
  Combining~\eqref{eq:case-2-max-u} and~\eqref{eq:case-2-min-u}, we realize that
  \begin{align*}
    I_1(\vw, \vx) &= \one{\exists \vxp \in \mB_0(\vx, k): \sgn(\langle \vw, \vxp \rangle_k) \neq \sgn(\langle \vw, \vx \rangle_k)} \\
                  &= \one{\sgn(    \max\{\langle \vw, \vxp \rangle_k: \vxp \in \mB_0(\vx, k)\}) \neq \sgn(    \min\{\langle \vw, \vxp \rangle_k: \vxp \in \mB_0(\vx, k)\})} \\
                  &= \one{\sgn(u_{(2k+1)} + \dots + u_{(d)}) \neq \sgn(u_{(1)} + \dots + u_{(d-2k)})} \\
    &= I_2(\vw, \vx).
  \end{align*}

  \underline{Case 3: $u_{i_{k+1}} = u_{i_{d-k}}= 0$.} Note that in this case, we
  have $u_{i_{k+1}} = \dots = u_{i_{d-k}} = 0$ and 
  \begin{equation*}
    \langle  \vw, \vx \rangle_k = u_{(k+1)} + \dots + u_{(d-k)} = u_{i_{k+1}} + \dots + u_{i_{d-k}} = 0.
  \end{equation*}
  Thereby,
  \begin{equation}
    \label{eq:case-3-I1-I3-simp}
    I_1(\vw, \vx) = \one{\exists \vxp \in \mB_0(\vx, k): \langle \vw, \vxp \rangle_k < 0} =: I_3(\vw, \vx).
  \end{equation}
  On the other hand, $u_{i_{k+1}} = 0$ implies $u_{i_j} \geq 0$ for $j \geq
  k+1$. Therefore
  \begin{equation*}
    u_{(2k+1)} + \dots + u_{(d)} \geq 0.
  \end{equation*}
  Hence, we have
  \begin{equation}
    \label{eq:case-3-I2-I4-simp}
    \begin{aligned}
      I_2(\vw, \vx) &= \one{\sgn(u_{(1)}+ \dots + u_{(d-2k)}) \neq \sgn(u_{(2k+1)} + \dots u_{(d)})} \\
      &= \one{\sgn(u_{(1)}+ \dots + u_{(d-2k)}) \neq 1} \\
      &= \one{u_{(1)}+ \dots + u_{(d-2k)} < 0} \\
      &=:I_4(\vw, \vx).
    \end{aligned}
  \end{equation}
  Combining~\eqref{eq:case-3-I1-I3-simp} and \eqref{eq:case-3-I2-I4-simp}, we
  realize that in order to show $I_1(\vw, \vx) = I_2(\vw, \vx)$, it suffices to
  show $I_3(\vw, \vx) = I_4(\vw, \vx)$. We verify this by considering 3 cases:
  \begin{itemize}
  \item   Assume that $I_4(\vw, \vx) = 0$.
    Then, using Lemma~\ref{lem:inf-sup-w-x-k-equality-cond}, we have
  \begin{equation*}
    \inf\{\langle \vw, \vxp \rangle_k: \vxp \in \mB_0(\vx, k)\} \geq u_{(1)} + \dots + u_{(d-2k)} \geq 0.
  \end{equation*}
  This means that for all $\vxp \in \mB_0(\vx, k)$, we have $\langle  \vw, \vxp
  \rangle_k \geq 0$ and $I_3(\vw, \vx) = 0 = I_4(\vw, \vx)$. 
\item Assume that $I_4(\vw, \vx) = 1$ and $|\{i: u_i \geq 0, w_i \neq 0\}| \geq
  k$. Then, from Lemma~\ref{lem:inf-sup-w-x-k-equality-cond}, we have
  \begin{equation*}
    \min\{\langle \vw, \vxp \rangle_k: \vxp \in \mB_0(\vx, k)\} = u_{(1)} + \dots +u_{(d-2k)}.  
  \end{equation*}
  Consequently, we have
  \begin{align*}
    I_3(\vw, \vx) &= \one{\exists \vxp \in \mB_0(\vx, k): \langle \vw, \vxp \rangle_k < 0} \\
                  &= \one{    \min\{\langle \vw, \vxp \rangle_k: \vxp \in \mB_0(\vx, k)\} < 0} \\
                  &= \one{u_{(1)} + \dots +u_{(d-2k)} < 0} \\
                  &= I_4(\vw, \vx).
  \end{align*}
\item Assume that $I_4(\vw, \vx) = 1$ and $|\{i: u_i \geq 0, w_i \neq 0\}| <
  k$. Note that by assumption of the lemma, we have $|\{i \in [d]: w_i \neq 0\}|
  > k$. We may write
  \begin{equation*}
    |\admiss_{\vw}| = |\{i \in [d]: w_i \neq 0\}| = |\admiss_{\vw}^+| + |\admiss_{\vw}^-|,
  \end{equation*}
  where
  \begin{align*}
    \admiss_{\vw}^+ &:= \{i \in [d]: u_i \geq 0, w_i \neq 0\} \\
    \admiss_{\vw}^- &:= \{i \in [d]: u_i < 0, w_i \neq 0\}.
  \end{align*}
  Since $|\admiss_{\vw}^+| < k$ and $|\admiss_{\vw}^+| + |\admiss_{\vw}^-| > k$,
  we have $|\admiss_{\vw}^-| > 0$.
  % This implies that there exists $i_* \in [d]$
  % such that $u_{i_*} < 0$ and $w_{i_*} \neq 0$.
  Now, we construct $\vxp \in
  \mB_0(\vx, k)$ as
  \begin{equation*}
    x'_i =
    \begin{cases}
      -w_i & i \in \admiss_{\vw}^+ \\
      x_i & \text{otherwise}.
    \end{cases}
  \end{equation*}
  Note that $|\admiss_{\vw}^+| < k$ guarantees that $\vxp \in \mB_0(\vx, k)$.
  Let $\vup := \vw \odot \vxp$ and note that for $i \in \admiss_{\vw}^+$, $u'_i
  = w_i x'_i = - w_i^2$. But $w_i \neq 0$ for $i \in \admiss_{\vw}^+$. Therefore, $u'_i <
  0$ for $i \in \admiss_{\vw}^+$. On the other hand, for $i \in
  \admiss_{\vw}^-$, we have $u'_i = u_i < 0$. Furthermore, for $i \in [d]
  \setminus \admiss_{\vw}$, we have $u'_i = u_i = w_i x_i = 0$. To sum up, we
  showed that for $i \in \admiss_{\vw} = \admiss_{\vw}^+ \cup \admiss_{\vw}^-$,
  we have $u'_i < 0$, and for $i \notin \admiss_{\vw}$, we have $u'_i = 0$. Note
  that $|\admiss_{\vw}| > k$. This means that there at least $k+1$ negative
  coordinates in $\vup$, and the remaining of the coordinates are zero.
  Therefore, at least one negative value  will survive after truncating the
  bottom $k$ coordinates in $\vup$, plus perhaps some other negative and some
  other zero values. Hence,
  \begin{equation*}
    \langle \vw, \vxp \rangle_k = \tsum_k(\vup) < 0.
  \end{equation*}
  Consequently, we have
  \begin{equation*}
    I_3(\vw, \vx) = \one{\exists \vxp \in \mB_0(\vx, k): \langle \vw, \vxp \rangle_k < 0} = 1 = I_4(\vw, \vx).
  \end{equation*}
\end{itemize}
To sum up, we showed that $I_3(\vw, \vx) = I_4(\vw, \vx)$ in all the cases, and
hence $I_1(\vw, \vx) = I_2(\vw, \vx)$ as was discussed above.

\underline{Case 4: $u_{i_{k+1}} \geq 0$ and $u_{i_{d-k}} > 0$.} We have
\begin{equation*}
  \langle \vw, \vx \rangle_k = \tsum_k(\vw \odot \vx) = u_{i_{k+1}} + \dots + u_{i_{d-k}} > 0.
\end{equation*}
This means that
\begin{equation}
  \label{eq:case-4-I1-exists-negative}
  I_1(\vw, \vx) = \one{\exists \vxp \in \mB_0(\vx, k): \langle \vw, \vx \rangle_k < 0}.
\end{equation}
On the other hand, since $u_{i_{d-k}} > 0$, for $j \geq d-k$, we have $u_{i_j}
\geq u_{i_{d-k}} > 0$. Since $u_i = w_i x_i$, this means that for $d-k \leq j
\leq d$, we have $u_{i_j} \geq 0$ and $w_{i_j} \neq 0$. Thereby
\begin{equation*}
  |\{i\in [d]: u_i \geq 0, w_i \neq 0\}| \geq |\{i_{d-k+1}, \dots, i_d\}| = k.
\end{equation*}
Consequently, Lemma~\ref{lem:inf-sup-w-x-k-equality-cond} implies that
\begin{equation*}
  \min\{\langle \vw, \vxp \rangle_k: \vxp \in \mB_0(\vx, k)\} = u_{(1)} + \dots + u_{(d-2k)}.
\end{equation*}
Combining this with~\eqref{eq:case-4-I1-exists-negative}, we have
\begin{equation}
  \label{eq:case-4-I1-one-1-d-2k-negative}
  I_1(\vw, \vx) = \one{u_{(1)} + \dots u_{(d-2k)} < 0}.
\end{equation}
Furthermore, for $j \geq 2k+1$, we have $u_{i_j} \geq u_{i_{k+1}} \geq 0$. This
means that $u_{(2k+1)} + \dots + u_{(d)} \geq 0$. Using this
in~\eqref{eq:case-4-I1-one-1-d-2k-negative} above, we realize that
\begin{equation*}
  I_1(\vw, \vx) = \one{\sgn(u_{(1)} + \dots + u_{(d-2k)}) \neq \sgn(u_{(2k+1)} + \dots + u_{(d)})} = I_2(\vw, \vx).
\end{equation*}
Consequently, we verified that $I_1(\vw, \vx) = I_2(\vw, \vx)$ in all the four
cases. This completes the proof.
\end{proof}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main_cal"
%%% End:

